Managing Networked IoT Assets Using Practical and Scalable Traffic Inference

The Internet has recently witnessed unprecedented growth of a class of connected assets called the Internet of Things (IoT). Due to relatively immature manufacturing processes and limited computing resources, IoTs have inadequate device-level security measures, exposing the Internet to various cyber risks. Prior research leveraged predictable patterns in IoT network traffic to develop inference models. However, they fall short of expectations in addressing practical challenges, preventing them from being deployed in production settings. This thesis identifies four practical challenges and develops techniques to address them which can help secure businesses and protect user privacy against growing cyber threats. My first contribution balances prediction gains against computing costs of traffic features for IoT traffic classification and monitoring. My second contribution addresses the challenges of measurement costs and data quality. I develop an inference method that uses stochastic and deterministic modeling to predict IoT devices in home networks from opaque and coarse-grained IPFIX flow data. Evaluations show that false positive rates can be reduced by 75% compared to related work without significantly affecting true positives. My third contribution focuses on the challenge of concept drifts by analyzing over six million flow records collected from 12 real home networks. Finally, my fourth contribution studies the resilience of machine learning models against adversarial attacks with a specific focus on decision tree-based models.

==> tex/acknowledgement.tex <==
\chapter*{Acknowledgment}
	\bookmarksetupnext{level=section}
	\addcontentsline{toc}{chapter}{Acknowledgment}
	\onehalfspace
	\bookmarksetupnext{level=section}

	Pursuing a Ph.D. degree is...
	
	I first and foremost thank ...
	
\onehalfspace

\vspace{-8mm}



\onehalfspace
\cleardoublepage
